LB Scalability: Achieving the Right Balance Between Being Stateful and Stateless

A high performance Layer-4 load balancer (LB) is one of the most important components of a cloud service infrastructure. Such an LB uses network and transport layer information for deciding how to distribute client requests across a group of servers. A crucial requirement for a stateful LB is per connection consistency (PCC); namely, that all the packets of the same connection will be forwarded to the same server, as long as the server is alive, even if the pool of servers or the assignment function changes. The challenge is in designing a high throughput, low latency solution that is also scalable. This paper proposes a highly scalable LB, called Prism, implemented using a programmable switch ASIC. As far as we know, Prism is the first reported LB that can process millions of connections per second and hundreds of millions connections in total, while ensuring PCC. This is due to the fact that Prism forwards all the packets in hardware, even during server pool changes, while avoiding the need to maintain a hardware state per every active connection. We implemented a prototype of the proposed architecture and showed that Prism can scale to 100 million simultaneous connections, and can accommodate more than one pool update per second.

==> ECMP_hashing.tex <==
\subsubsection*{\textbf{ECMP table update process}}
Prior to the update process, each bin in the ECMP table holds some DIP pointer such that the load is distributed evenly, i.e. each DIP pointer appears the same number of times in the ECMP table. There are two basic update operations that should be defined; the removal of a DIP and the addition of a DIP. In the first operation, the removal of a DIP results in empty bins in the ECMP table. These bins must be updated with other pool DIPs to keep the ECMP table in a valid state and with uniform distribution. All bins must always have a valid DIP pointer since the packet header 5-tuple might be hashed to any of the bins in the ECMP table.

\subsubsection*{\textbf{Hashing algorithms for updating ECMP table}}
Consistent hashing \cite{karger1997consistent} is a widely used hashing scheme to minimize relocating objects in the ring. In our case, the ring is the ECMP table which is an array of size 128 and the objects are DIP pointers. When a DIP is removed from the table, its bins are filled with the first next right neighbour in the ring. When a DIP is added, a $\ceil*{\frac{128}{N}}$ bins are chosen randomly and the new DIP is inserted there. This way the load is distributed evenly between the DIPs of the pool, and in the DIP adding process only $\ceil*{\frac{128}{N}}$ bins are changed causing minimal disruption.
\par Resilient hashing \cite{matthews2013resilient} is another load balancing scheme used in layer-3 to minimize disruption of links update. The focus in resilient hashing is on the failure/removal of a link, in such case the hash distribution scheme will be redefined such that the unaffected flows will not be reassigned to new links and the affected flows will be redistributed across the remaining links. Resilient hashing does not guarantee that adding links will preserve mappings of old flows, i.e. old flows might go through different link from previously. The ECMP mechanism available in switches has a resilient hashing mode \cite{ECMP}. In this mode a fixed number of hash buckets are defined which are equivalent to bins in our context. Each bucket points to a next hop which are equivalent to DIPs in our context. If a next hop is removed from the pool, the number of buckets does not change, unlike default ECMP hashing. The empty buckets are assigned with next hops in a round robin fashion. If a next hop is added to the pool, the whole buckets might change to distribute the load evenly, this handling is different from consistent hashing. For our system we would use a combination of both hashing schemes to choose bins.




==> broken_connection_figure.tex <==
\begin{figure*}[h!]
\centering
\begin{minipage}[b]{.4\textwidth}
\scalebox{0.45}{\input{simulation_figures/broken_connections_36_bit.pgf}}
\caption*{\small \textmd{(a) 36-bits signature length, $\Delta$ = 5 seconds}}
\end{minipage}\qquad \qquad
\begin{minipage}[b]{.4\textwidth}
\scalebox{0.45}{\input{simulation_figures/broken_connections_40_bit.pgf}}
\caption*{\small \textmd{(b) 40-bits signature length, $\Delta$ = 5 seconds}}
\end{minipage}
\caption{ \centering The number of broken connections throughout system running time, as a function of SYN arrival rate for a single VIP}
\label{fig:broken_connections}
\end{figure*}

 Figure~\ref{fig:broken_connections} present simulation results for a VIP for which the connection arrival rate varies between 10,000 to 50,000 per second, the frequent update happens every 10 seconds, the number of DIPs is 100 and each DIP resides in one bin, and the average connection length is 100 seconds. The signature length is a parameter of this experiment. The objective of the experiment is to verify that dropping those SYNs is legitimate, and practically no connections are broken. As seen in Figure~\ref{fig:broken_connections}(a), using 36-bit signature will result in broken connections, but with 40-bit signature the number of broken connections drops drastically. Figure~\ref{fig:broken_connections}(b) shows that with 10,000 SYN arrival rate no connections are broken. Since we use in our prototype a 48-bit signature under a VIP, having a broken connection due to the above assumption is practically not possible.

==> choosing_ecmp_bins.tex <==
\subsection{Choosing ECMP bins}
The chosen bins to be updated directly affect the time required to complete the migration process. Therefore, it is desired to choose bins with fewer connections. Another factor to be considered is the limited capacity of the MCT. The MCT should not hold connections for a long period, because this would hurt its insertion latency and consequently delay the migration process. So it is not accurate to prefer choosing bins with fewer connections. A better indicator is the life expectancy (LE) of the connections, defined as the average life of a connection of the VIP minus the active time of the connection. If the total life expectancy under a bin is lower, then the migration of the bin would produce less load on the MCT. As mentioned earlier in the paper, there might be more than one active connection associated with a SIG. The LE of a SIG is calculated according to the latest connection, e.g. inserting a new connection with the same SIG would make the active time of the SIG equal to zero. 
\par We define the load of a bin as:  $$W(bin) = {\sum_{SIG \in bin} LE(SIG)}$$
For example, suppose we have two bins: bin1 with SIG1 and SIG2 such that LE(SIG1)=LE(SIG2)=2, bin2 with SIG3 such that LE(SIG3)=5. By the above metric, bin1 would be preferred over bin2 to be migrated.

$$(W(bin) = {\alpha \cdot \sum_{SIG \in bin} LE(SIG) + (1-\alpha)\cdot|bin|})$$

==> dynamic_ecmp_sizing.tex <==
\subsection{Dynamic ECMP sizing}
Hardware storage usage is also dependant on ECMP table size. Reducing the ECMP size for VIPs means that more SIGs can fit into the MCT or the FIB. Larger ECMP lowers the number of connections under each bin, so migrating a bin would take less time. In a larger ECMP a DIP would appear in more bins; proportional to its processing power in the VIP. The total number of connections a DIP handles for a VIP would still be proportional to its processing power, regardless of the size of the ECMP table.
\par
The ECMP size should be close to $K\cdot|Pool|$. Having a very big ECMP does not benefit performance, so $K$ should be a small constant. The minimal size is when $K=1$, in this case, the ECMP table must be expanded before adding a DIP to the pool. We would use the popular method where the growth factor is 2, i.e. the table size is doubled. The new bins are filled with the available DIPs. This is illustrated in Figure~\ref{fig:ecmp_expand}.

\input{ecmp_size_expanding_figure.tex}


==> ecmp_update_figure.tex <==

\begin{tikzpicture}[node distance = 3cm, auto]

\end{tikzpicture}
\caption{\centering Adding a new DIP (DIP5) to a certain VIP}
\label{fig:ecmp_update_new}

==> fib_collision_figure.tex <==
\begin{figure}[t]
\scalebox{0.45}{\input{simulation_figures/syns_collisions_new1.pgf}}
\caption{\centering The number of collisions in the FIB(SYN) table, as a function of the number of received SYNs and signature length}
\label{fig:SYNs_vs_Collisions}
\end{figure}

==> fib_table.tex <==

\par FIB entry insertion is done by hardware with the arrival of SYN/FIN packets. First, the relevant table is chosen according to the packet destination and SYN/FIN bits in the header. The type of entry can be SYN or FIN. Figure \ref{fib_table_id} illustrates the table ID which is used to access the FIB table; bit 0 is set for tables of SYN entries, and is unset for tables of FIN entries. The other 15 bits identifies the VIP of the packet. The FIB can be seen as a table of tables such that each table holds SYN/FIN connection signatures of a specific VIP.

\begin{figure}[h!]
\begin{center}
\begin{bytefield}[bitwidth=1.25em]{16}
  \bitheader{0-15} \\
  \bitbox{1}{\tiny S/F}
  \bitbox{15}{\tiny VIP ID}
\end{bytefield}
\end{center}
\caption{\centering 16-bit table ID consists of 1-bit for SYN/FIN bit and 15-bit for VIP}
\label{fib_table_id}
\end{figure}



%\begin{figure}[h!]
%\begin{tabular}{|p{2cm} | p{2cm}|}
%    \hline
%    \multicolumn{1}{|p{2cm}|}{\centering SMAC} & \multicolumn{1}{|p{2cm}|}{\centering DMAC}\\
%    \hline
%    \multicolumn{1}{c}{\upbracefill} & \multicolumn{1}{c}{\upbracefill}\\[-0.5ex]
%    \multicolumn{1}{c}{\small 48-bit packet SIG} & \multicolumn{1}{c}{\small 48-bit VIP+port } 
%\end{tabular}
%\caption{MAC learning}
%\end{figure}

==> mac_learning_figure.tex <==
\begin{figure}[hb!]
\begin{tabular}{|p{2cm} | p{2cm}|}
    \hline
    \multicolumn{1}{|p{2cm}|}{\centering SMAC} & \multicolumn{1}{|p{2cm}|}{\centering DMAC}\\
    \hline
    \multicolumn{1}{c}{\upbracefill} & \multicolumn{1}{c}{\upbracefill}\\[-0.5ex]
    \multicolumn{1}{c}{\small 48-bit packet SIG} & \multicolumn{1}{c}{\small 48-bit VIP+port } 
\end{tabular}
\caption{MAC learning}
\label{fig:mac learning}
\end{figure}

==> mct_figure.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{ | c | c | } 
  \hline
  migrated connection key & DIP \\
  \hlineB{2.5}
  conn1-key & DIP1  \\
  \hline
  conn3-key & DIP3  \\ 
  \hline
\end{tabular}
\end{center}
\caption{Migrated connections table}
\centering \footnotesize The pool update process changed bin125 and bin43, so connections 1 and 3 were copied to the MCT with their old bin values
\end{table}

==> sct_figure.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{ | c | c | } 
  \hline
  connection key & DIP \\
  \hlineB{2.5}
  conn1-key & DIP1  \\
  \hline
  conn2-key & DIP2  \\
  \hline
  conn3-key & DIP3  \\ 
  \hline
  conn4-key & DIP4  \\ 
  \hline
\end{tabular}
\end{center}
\caption{Full connections table}
\centering \footnotesize connections are mapped according to the ECMP table as follows: \newline $bin125 \rightarrow DIP1$, $bin2 \rightarrow DIP2$,  $bin43 \rightarrow DIP3$,  $bin84 \rightarrow DIP4$
\end{table}

==> signature_collisions_section.tex <==
\section{Connection Signature}
\label{sec:signatures}

Memory usage for FIB and MCT is mainly dependent on the length of the connection match key. To reduce the consumption of expensive hardware storage, Prism does not remember the whole 5-tuple of the connections. Instead, the 5-tuple, or part of it, is used for computing a connection signature for each connection.

\par Using signatures introduces collisions. We actually may have two types of collisions. The first is that two different connections, with different 5-tuples, are hashed to different signatures, but these two signatures are  mapped to the same cuckoo table entry. The second type is that two different connections, with different 5-tuples, happen to have the same signature. 

\par The first type of collisions is resolved using standard cuckoo hashing techniques \cite{pagh2004cuckoo,bosshart2013forwarding}. Namely, a signature that hits an occupied hash entry is mapped to another cuckoo stage with a different hash function. Hence, from now on we address only collisions from the second type. 

\par Prism uses a 48-bit connection signature (Figure~\ref{fig:signature}). This length was chosen for two reasons, the first is to leverage the L2 hardware MAC learning, which learns the 48-bit source MAC addresses of Ethernet frames. The second reason is reducing collision probability. The signature consists of 24-bit hash of the 5-tuple connection key; this partition is employed due to hardware hash limitations which limits the generated hash size to 24-bit. The definition of the other 24 bits impacts the implementation choice of MCT and FIB.   

\input{signature_figure.tex}
We now describe two options for defining the first part of the signature. The first option is to take 16-bit for destination VIP ID, and additional 8 bits from the source port number. The second option is to take 16 bits from the source IP address and additional 8 bits from the source port number. The main differences between the two options are as follows:
\begin{enumerate}
\item If the first option is used, it is enough to maintain one FIB table for all the connections. If the second option is used, we need to maintain a FIB table for each VIP, in order to keep the VIP information in the SCT.

\item If the first option is used, an ECMP table has to be maintained for each VIP, or equivalently, the VIP is used together with the signature in order to choose the right ECMP bin (see Figure 1). 

\item If the first option is used, then two different connections with the same signatures are destined for the same VIP; namely, \newline $\text{SIG(conn1-key)} = \text{SIG(conn2-key)} \Rightarrow \text{VIP1 = VIP2}.$ This implies that they are also mapped to the same ECMP bin. Hence, if one of them is migrated from bin i to bin j, the other is also migrated from bin i to bin j. However, if the second option is used, then the above property can not be concluded. Therefore, we actually need to maintain an MCT per each VIP.
\end{enumerate}

\par
SCT is where we manage collided signatures, reference counting technique would count the number of active connections that are mapped to the same signature. Tracking the number of active connections hashed to each signature is necessary in order to clear unused signatures properly; a signature is cleared only when all connections hashed to it were closed. Figure~\ref{fig:all tables} presents our architecture tables after the introduction of signatures and reference counting.

\subsection{Collision Scenarios}
\par We need to distinguish between two collision scenarios: a) A SYN is received for a given signature when a connection with the same signature is already in the SCT; b) A SYN is received for a given signature when a connection with the same signature is still in the FIB(SYN). In the first case, the collision would be resolved by incrementing the counter of the SCT entry after fetching the signature from the FIB(SYN). In the second case, the SYN packet is triggered to be handled by the software as shown in Figure~\ref{entry_insertion_figure}, otherwise the signature would be lost. Note, the second scenario can not be resolved by reference counting since it is not available in the FIB. We show in Section~\ref{sec:analysis} that this case is very rare, and therefore not worth sacrificing hardware storage for integrating reference counting in the FIB.

\par For example, as seen in SCT in Figure~\ref{fig:all tables}, the signatures of conn2 and conn4 are equal so they are put in the same entry in the SCT with reference count of value 2. This collision is of the second type, and it could have resulted from scenario (a) or (b).


==> tables_signature_figure.tex <==
\begin{figure*}[ht!]

\begin{subfigure}
\begin{tabular}{ | c | c | c | c | } 
  \hline
  \multicolumn{4}{|c|}{SCT} \\
  \hline
  connection signature & DIP & bin & ref counter\\
  \hlineB{2.5}
  SIG(conn1-key) & DIP1 & bin1 & 1 \\
  \hline
  SIG(conn2-key) & DIP2 & bin2 & 2 \\
  \hline
  SIG(conn3-key) & DIP3 & bin3 & 1 \\ 
  \hline
\end{tabular}
%\centering \footnotesize connection conn2 and conn4 hash digest to the same signature
\end{subfigure}
\centering
\begin{subfigure}
\begin{tabular}{ | c | }
  \hline
  \multicolumn{1}{|c|}{FIB(SYN/FIN)} \\
  \hline
  new connection key \\
  \hlineB{2.5}
   SIG(conn1-key)  \\
  \hline
  SIG(conn2-key)  \\
  \hline
  SIG(conn3-key)  \\ 
  \hline
  SIG(conn4-key)   \\ 
  \hline
\end{tabular}
\end{subfigure}
\centering
\begin{subfigure}
\begin{tabular}{ | c | c | } 
  \hline
  \multicolumn{2}{|c|}{MCT} \\
  \hline
  migrated connection key & DIP \\
  \hlineB{2.5}
  SIG(conn1-key) & DIP1  \\
  \hline
  SIG(conn3-key) & DIP3  \\ 
  \hline
\end{tabular}
\end{subfigure}

\caption{Our tables after introducing connection SIG}
\label{fig:all tables}
\end{figure*}

==> transitTable.tex <==
\par Our LB ensures PCC by copying all affected connections to MCT before updating the ECMP table. This is equivalent to SilkRoad's use of TransitTable to detect affected connections and select the correct DIP for them from the DIPPoolTable. In our LB this DIP will already be in the MCT, and no further table accesses are needed. Packets of old connections which their bin was affected will hit on the MCT and pick the DIP from it. All other packets will pick their DIP according to the ECMP table. This way all packets will be forwarded correctly ensuring PCC. Unlike SilkRoad we do not need to save several versions of each DIP pool to ensure PCC. But the pool update and connections migration should be done efficiently as we show in Section~\ref{sec:dip pool update}.
